Towards Lifelong Learning of Large Language Models: A Survey

As the applications of large language models (LLMs) expand across diverse fields, the ability of these models to adapt to ongoing changes in data, tasks, and user preferences becomes crucial. Traditional training methods, relying on static datasets, are increasingly inadequate for coping with the dynamic nature of real-world information. Lifelong learning, also known as continual or incremental learning, addresses this challenge by enabling LLMs to learn continuously and adaptively over their operational lifetime, integrating new knowledge while retaining previously learned information and preventing catastrophic forgetting. This survey delves into the sophisticated landscape of lifelong learning, categorizing strategies into two primary groups: Internal Knowledge and External Knowledge. Internal Knowledge includes continual pretraining and continual finetuning, each enhancing the adaptability of LLMs in various scenarios. External Knowledge encompasses retrieval-based and tool-based lifelong learning, leveraging external data sources and computational tools to extend the model's capabilities without modifying core parameters. The key contributions of our survey are: (1) Introducing a novel taxonomy categorizing the extensive literature of lifelong learning into 12 scenarios; (2) Identifying common techniques across all lifelong learning scenarios and classifying existing literature into various technique groups within each scenario; (3) Highlighting emerging techniques such as model expansion and data selection, which were less explored in the pre-LLM era. Through a detailed examination of these groups and their respective categories, this survey aims to enhance the adaptability, reliability, and overall performance of LLMs in real-world applications.

==> tables/RE_MT_methods.tex <==
\begin{tabular}{llllllllllll}
    \toprule
    \multicolumn{1}{c}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{Year}} & \multicolumn{1}{c}{\textbf{Publication}} & \multicolumn{1}{c}{\textbf{Backbone}} & \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Code}} & \multicolumn{1}{c}{\textbf{PEFT}} & \multicolumn{1}{c}{\textbf{Replay}} & \multicolumn{1}{c}{\textbf{Distillation}} & \multicolumn{1}{c}{\textbf{Regularization}} & \multicolumn{1}{c}{\textbf{Architecture}} & \multicolumn{1}{c}{\textbf{Others}} \\
    \midrule
    \rowcolor[rgb]{ .788,  .788,  .788} \multicolumn{12}{c}{\textit{\textbf{Continual Relation Extraction}}} \\
    \midrule
    \rowcolor[rgb]{ 1,  .949,  .8} ConPL \cite{chen2023consistent} & 2023  & ACL   & BERT  & FewRel, TACRED & \href{https://github.com/XiudiChen/ConPL}{Link} & Prompt Tuning & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & Prototype \\
    \midrule
    Xia et. al \cite{xia2023enhancing} & 2023  & ACL (Findings) & BERT  & FewRel, TACRED & \href{https://github.com/hemingkx/CDec}{Link} & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & Adversarial Tuning \\
    \midrule
    \rowcolor[rgb]{ 1,  .949,  .8} CEAR \cite{CEAR} & 2023  & ACL   & BERT  & FewRel, TACRED & \href{https://github.com/nju-websoft/CEAR}{Link} & /     & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & Contrastive Learning, Prototype \\
    \midrule
    SCKD \cite{SCKD} & 2023  & ACL (Findings) & BERT  & FewRel, TACRED & \href{https://github.com/nju-websoft/SCKD}{Link} & /     & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & /     & Data Augmentation \\
    \midrule
    \rowcolor[rgb]{ 1,  .949,  .8} ICE \cite{liu2023teamwork} & 2023  & ACL (Findings) & BERT  & TACRED & \href{https://github.com/VT-NLP/ICE}{Link} & /     & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & Frozen Backbones \\
    \midrule
    ICA-Proto \cite{jiang2023ica} & 2023  & EACL (Findings) & BERT, Glove & FewRel & /     & /     & /     & /     & /     & /     & Prototype \\
    \midrule
    \rowcolor[rgb]{ 1,  .949,  .8} SEQ* \cite{zheng2023learn} & 2024  & ACL   & BERT, GPT2, Pythia & FewRel, TACRED & \href{https://github.com/zzz47zzz/codebase-for-incremental-learning-with-llm}{Link} & /     & /     & /     & /     & /     & Classifier Expasion \\
    \midrule
    \rowcolor[rgb]{ .788,  .788,  .788} \multicolumn{12}{c}{\textit{\textbf{Continual Machine Translation}}} \\
    \midrule
    \rowcolor[rgb]{ .886,  .937,  .855} CKD \cite{zhang2023continualknowledge} & 2023  & ACL   & Transformer & LDC,  TED transcripts, Subtitles & \href{https://github.com/THUNLP-MT/CKD}{Link} & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & / \\
    \midrule
    KT \cite{huang2023knowledge} & 2023  & ACL   & Transformer & WMT   & \href{https://github.com/THUNLP-MT/ktnmt}{Link} & /     & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    \rowcolor[rgb]{ .886,  .937,  .855} BVP \cite{liu2023continual} & 2023  & EMNLP & mBART50-nn & WMT   & \href{https://github.com/raburabu91/BVP4CL}{Link} & /     & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & Pruning \\
    \midrule
    F-MALLOC \cite{wu2024f} & 2024  & NAACL & Transformer & WMT   & \href{https://github.com/WJMacro/ContinualMT.}{Link} & /     & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & Pruning \\
    \bottomrule
\end{tabular}%

==> tables/TC_NER_methods.tex <==
\begin{tabular}{llllllllllll}
    \toprule
    \multicolumn{1}{c}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{Year}} & \multicolumn{1}{c}{\textbf{Publication}} & \multicolumn{1}{c}{\textbf{Backbone}} & \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Code}} & \multicolumn{1}{c}{\textbf{PEFT}} & \multicolumn{1}{c}{\textbf{Replay}} & \multicolumn{1}{c}{\textbf{Distillation}} & \multicolumn{1}{c}{\textbf{Regularization}} & \multicolumn{1}{c}{\textbf{Architecture}} & \multicolumn{1}{c}{\textbf{Others}} \\
    \midrule
    \rowcolor[rgb]{ .788,  .788,  .788} \multicolumn{12}{c}{\textit{\textbf{Continual Text Classification}}} \\
    \midrule
    \rowcolor[rgb]{ .867,  .922,  .969} EPI \cite{wang2023rehearsal} & 2023  & ACL   & BERT  & AGNews, Yelp, Amazon, DBPedia, Yahoo, WOS & \href{https://github.com/Dicer-Zz/EPI}{Link} & Prefix Tuning & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    VAG \cite{shao2023class} & 2023  & ACL   & BART  & CLINC150, BANKING77, 20 Newsgroups & \href{https://github.com/shaoyijia/VAG}{Link} & /     & Label-based Pseudo Replay & /     & /     & /     & Vocabulary \\
    \midrule
    \rowcolor[rgb]{ .867,  .922,  .969} LR ADJUST \cite{winata2023overcoming} & 2023  & ACL (Findings) & XLM-R & MASSIVE, WikiAnn & /     & /     & /     & /     & /     & /     & Adjusts Learning Rate \\
    \midrule
    InfoCL \cite{song2023infocl} & 2023  & EMNLP & BERT  & HWU64, FewRel, TACRED, MAVEN,  & \href{https://github.com/Yifan-Song793/InfoCL}{Link} & /     & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & Contrastive Learning \\
    \midrule
    \rowcolor[rgb]{ .867,  .922,  .969} MoCL \cite{wang2024rehearsal} & 2024  & NAACL & BERT, T5, LLaMA & WOS, AGNews, Yelp, Amazon, DBPedia, Yahoo & \href{https://github.com/boschresearch/MoCL-NAACL-2024}{Link} & LoRA, Prefix Tuning & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    SEQ* \cite{zheng2023learn} & 2024  & ACL   & BERT, GPT2, Pythia & AGNews, Yelp, Amazon, DBPedia, Yahoo & \href{https://github.com/zzz47zzz/codebase-for-incremental-learning-with-llm}{Link} & /     & /     & /     & /     & /     & Classifier Expasion \\
    \midrule
    \rowcolor[rgb]{ .788,  .788,  .788} \multicolumn{12}{c}{\textit{\textbf{Continual Named Entity Recognition}}} \\
    \midrule
    \rowcolor[rgb]{ .988,  .894,  .839} SpanKL \cite{zhang2023neural} & 2023  & AAAI  & BERT  & OntoNotes5, Few-NERD & \href{https://github.com/Qznan/SpanK}{Link} & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & Span-Level Prediction \\
    \midrule
    OCILNER \cite{ma2023learning} & 2023  & ACL   & BERT  & CoNLL 2003, OntoNotes5, Few-NERD & \href{https://github.com/rtmaww/O_CILNER}{Link} & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & Contrastive Learning, Prototype \\
    \midrule
    \rowcolor[rgb]{ .988,  .894,  .839} ICE \cite{liu2023teamwork} & 2023  & ACL Findings & BERT  & Few-NERD, MAVEN, ACE 2005 & \href{https://github.com/VT-NLP/ICE}{Link} & /     & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & Frozen Backbones \\
    \midrule
    RDP \cite{zhang2023task} & 2023  & CIKM  & BERT  & CoNLL 2003, OntoNotes5, I2B2 & \href{https://github.com/BladeDancer957/INER_RDP}{Link} & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & Prototype \\
    \midrule
    \rowcolor[rgb]{ .988,  .894,  .839} CPFD \cite{zhang2023continual} & 2023  & EMNLP & BERT  & CoNLL 2003, OntoNotes5, I2B2 & \href{https://github.com/BladeDancer957/CPFD}{Link} & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & /     & / \\
    \midrule
    SKD-NER \cite{chen2023skd} & 2023  & EMNLP & BERT  & OntoNotes5, Few-NERD & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & Reinforcement Learning \\
    \midrule
    \rowcolor[rgb]{ .988,  .894,  .839} Liang et. al. \cite{liang2023novel} & 2023  & EMNLP (Findings) & BERT  & ATIS, Snips & \href{https://github.com/cs-liangchen-work/NovelIE}{Link} & /     & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & Prototype \\
    \midrule
    DLD \cite{zhang2023decomposing} & 2023  & SIGIR & BERT  & CoNLL 2003, OntoNotes5, I2B2 & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & / \\
    \midrule
    \rowcolor[rgb]{ .988,  .894,  .839} IS3 \cite{qiu2024incremental} & 2024  & ACL (Findings) & BERT  & OntoNotes5, I2B2, MAVEN & \href{https://github.com/zzz47zzz/codebase-for-incremental-learning-with-llm}{Link} & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & / \\
    \midrule
    SEQ* \cite{zheng2023learn} & 2024  & ACL   & BERT, GPT2, Pythia & OntoNotes5, I2B2, Few-NERD & \href{https://github.com/zzz47zzz/codebase-for-incremental-learning-with-llm}{Link} & /     & /     & /     & /     & /     & Classifier Expasion \\
    \bottomrule
\end{tabular}

==> tables/task_agnostic_methods.tex <==
\begin{tabular}{llllllllllll}
        \toprule
    \multicolumn{1}{c}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{Year}} & \multicolumn{1}{c}{\textbf{Publication}} & \multicolumn{1}{c}{\textbf{Backbone}} & \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Code}} & \multicolumn{1}{c}{\textbf{PEFT}} & \multicolumn{1}{c}{\textbf{Replay}} & \multicolumn{1}{c}{\textbf{Distillation}} & \multicolumn{1}{c}{\textbf{Regularization}} & \multicolumn{1}{c}{\textbf{Architecture}} & \multicolumn{1}{c}{\textbf{Others}} \\
    \midrule
    \rowcolor[rgb]{ .788,  .788,  .788} \multicolumn{12}{c}{\textit{\textbf{Continual Instruction Tuning}}} \\
    \midrule
    ACM \cite{zhang2022continual} & 2022  & ACL   & GPT-2 & E2ENLG, RNNLG, WikiSQL, CNN/DailyMail, MultiWOZ & \href{https://github.com/GT-SALT/Adaptive-Compositional-Modules}{Link} & Adapters & Pseudo Sample & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} InstructionSpeak \cite{yin2022contintin} & 2022  & ACL   & BART  & NaturalInstructions & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & / \\
    \midrule
    Continual Prompt Tuning \cite{zhu2022continual} & 2022  & ACL   & T5    & Schema Guided Dialogue & \href{https://github.com/thu-coai/cpt4dst}{Link} & Prompt Tuning & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} PCLL \cite{zhao2022prompt} & 2022  & EMNLP & GPT-2 & DSTC, TOP & \href{https://github.com/AlibabaResearch/DAMO-ConvAI/tree/main/pcll}{Link} & /     & Pseudo Sample & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & Variational Auto Encoder \\
    \midrule
    CT0 \cite{scialom2022fine} & 2022  & EMNLP & T0    & Simpl, HGen, Haiku, CQA, InqQG, EmDg, Exp, TwSt & \href{https://github.com/ThomasScialom/T0_continual_learning}{Link} & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} LFPT5 \cite{qin2021lfpt5} & 2022  & ICLR  & T5    & AGNews, Amazon Review, DBPedia, Yahoo, CNNDM, WikiHow, Xsum & \href{https://github.com/qcwthu/Lifelong-Fewshot-Language-Learning}{Link} & Prompt Tuning & Pseudo Sample & /     & /     & /     & / \\
    \midrule
    LPT \cite{liang2023prompts} & 2023  & ACL   & T5    & CoNLL03, ACE05, SemEval-14 & \href{https://github.com/jokieleung/Lottery_Prompt}{Link} & Prompt Tuning & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & Pruning \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} DYNAINST \cite{mok2023large} & 2023  & ACL   & BART  & SuperNI & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & / \\
    \midrule
    HMI-LAMOL \cite{maekawa2023generative} & 2023  & EACL  & GPT-2, BERT & AGNews, Yelp, Amazon, DBPedia, Yahoo & \href{https://github.com/arumaekawa/GR-HMI}{Link} & /     & Pseudo Sample & /     & /     & /     & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} DMEA \cite{qin2023lifelong} & 2023  & EMNLP & GPT-2, BERT & CNN/DailyMail, MultiWOZ, WikiSQL & /     & Adapters & /     & /     & /     & /     & / \\
    \midrule
    O-LoRA \cite{wang2023orthogonal} & 2023  & EMNLP (Findings) & LLaMA, T5 & GLUE, SuperGLUE, IMDB & \href{https://github.com/cmnfriend/O-LoRA}{Link} & LoRA  & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & Orthogonal Subspaces \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} TSS \cite{ke2023sub} & 2023  & EMNLP (Findings) & BART  & AGNews, Yelp, Amazon, DBPedia, Yahoo & \href{https://github.com/ZixuanKe/PyContinual}{Link} & Adapters & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    ProgPrompt \cite{razdaibiedina2022progressive} & 2023  & ICLR  & T5, BERT & GLUE, SuperGLUE, IMDB & \href{https://github.com/arazd/ProgressivePrompts}{Link} & Prompt Tuning & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} SAPT \cite{modulesapt} & 2024  & /     & LLaMA, T5 & SuperNI, GLUE, SuperGLUE, IMDB & /     & Prompt Tuning, LoRA & Pseudo Sample & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    InsCL \cite{wang2024inscl} & 2024  & /     & LLaMA & SuperNI & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} I-LoRA \cite{ren2024analyzing} & 2024  & /     & LLaMA & ScienseQA, MedMCQA, BBH, PIQA & \href{https://github.com/which47/LLMCL}{Link} & LoRA  & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    SSR \cite{huang2024mitigating} & 2024  & /     & LLaMA, Alpaca & SuperNI & /     & LoRA  & Pseudo Sample & /     & /     & /     & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} SLM \cite{bohaoscalable} & 2024  & ICLR  & LLaMA, T5, BERT & AGNews, Yelp, Amazon, DBPedia, Yahoo & \href{https://github.com/Pbihao/SLM}{Link} & LoRA  & /     & /     & /     & /     & / \\
    \midrule
    Q-Tuning \cite{guo2024q} & 2024  & NAACL (Findings) & BERT, T5 & GLUE, SuperGLUE, IMDB & /     & Prompt Tuning & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    \rowcolor[rgb]{ .937,  .933,  .992} SAPT \cite{modulesapt} & 2024  & /     & T5, LLaMA & SuperNI, GLUE, SuperGLUE, IMDB & /     & LoRA, Prompt Tuning & Pseudo Sample & \color[RGB]{3,191,61}{\Checkmark} & \color[RGB]{3,191,61}{\Checkmark} & /     & / \\
    \midrule
    MoRAL \cite{moral} & 2024  & /     & LLaMA, Phi & Arxiv, HotpotQA & /     & LoRA  & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    \rowcolor[rgb]{ .788,  .788,  .788} \multicolumn{12}{c}{\textit{\textbf{Continual Knowledge Editing}}} \\
    \midrule
    \rowcolor[rgb]{ .992,  .937,  .878} SLAG \cite{SLAG} & 2023  & EACL  & BART, RoBERTa & zsRE, Wikidata5m, FEVER, LeapOfThought & \href{https://github.com/peterbhase/SLAG-Belief-Updating}{Link} & /     & /     & /     & /     & /     & / \\
    \midrule
    GRACE \cite{GRACE} & 2023  & ICLR  & T5, BERT & zsRE, SCOTUS, Natural Questions & /     & GRACE Adapters & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & Codebook \\
    \midrule
    \rowcolor[rgb]{ .992,  .937,  .878} TPatcher \cite{TPatcher} & 2023  & ICLR  & BART, BERT & zsRE, FEVER, CBQA & \href{https://github.com/ZeroYuHuang/Transformer-Patcher}{Link} & /     & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    WilKE \cite{WilKE} & 2024  & /     & GPT-J, GPT-2 & CounterFact & /     & /     & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & / \\
    \midrule
    \rowcolor[rgb]{ .788,  .788,  .788} \multicolumn{12}{c}{\textit{\textbf{Continual Alignment}}} \\
    \midrule
    Zhao et. al. \cite{zhao2023learning} & 2023  & /     & LLaMA, GPT-2 & BBQ, Pile, HarmfulQA & /     & LoRA  & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & /     & Data Filtering, Self-Correction \\
    \midrule
    \rowcolor[rgb]{ .839,  .863,  .894} CPPO \cite{zhangcppo} & 2024  & ICLR  & LLaMA, GPT-2 & HH-RLHF, Reddit TL;DR & \href{https://openi.pcl.ac.cn/Hanlard/CPPO}{Link} & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & /     & / \\
    \midrule
    COPR \cite{zhang2024copr} & 2024  & /     & LLaMA, GPT-J, OPT, & HH-RLHF, Reddit TL;DR, IMDB & \href{https://openi.pcl.ac.cn/Hanlard/Offline_alignment_methods_based_on_trlx.git}{Link} & /     & /     & /     & \color[RGB]{3,191,61}{\Checkmark} & /     & / \\
    \bottomrule
\end{tabular}%

==> tables/taxonomy_w_methods.tex <==
\tikzset{
        my node/.style={
            draw,
            align=center,
            thin,
            text width=1.2cm, 
            % minimum height=1cm,
            rounded corners=3,
        },
        my leaf/.style={
            draw,
            align=left,
            thin,
            % minimum width=1cm,
            text width=4.5cm, 
            % text height=1cm, 
            % minimum height=0.5cm,
            rounded corners=3,
        }
}
\forestset{
  every leaf node/.style={
    if n children=0{#1}{}
  },
  every tree node/.style={
    if n children=0{minimum width=1em}{#1}
  },
}
\begin{forest}
    for tree={%
        % my node,
        every leaf node={my leaf, font=\footnotesize},
        every tree node={my node, font=\small, l sep-=4.5pt, l-=1.pt},
        anchor=west,
        inner sep=2pt,
        % l = 10pt,
        l sep=10pt, % control leaf to parent nodes gaps (horizontal)
        s sep=5pt, % control node gaps (vertical)
        fit=tight,
        grow'=east,
        edge={ultra thin},
        parent anchor=east,
        child anchor=west,
        if n children=0{tier=last}{},
        edge path={
            \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(5pt,0) |- (.child anchor)\forestoption{edge label};
        },
        if={isodd(n_children())}{
            for children={
                if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
            }
        }{}
    }
    [\footnotesize Lifelong Learning of LLMs, draw=gray, color=gray!100, fill=gray!15, very thick, text=black 
        [\footnotesize Internal Knowledge, color=brightlavender!100, fill=brightlavender!15, very thick, text=black
            [\footnotesize Continual Pretraining \cref{sec:continual_pretraining}, color=cyan!100, fill=cyan!15, very thick, text=black
                [Continual Vertical Domain Pretraining \cref{sec:continual_vertical_domain_pretraining}, color=cyan!100, fill=cyan!15, very thick, text=black, tier=Task, text width=3.0cm
                    [ 
                        {
                             RHO-1 \cite{rho}, CorpusBrain++ \cite{corpusbrain}, Med-PaLM \cite{large}, ELLE \cite{elle}, Jin et al. \cite{Lifelongpretraining}, bert2BERT \cite{bert2bert}, LLaMA-Pro \cite{llama}, SOLAR \cite{solar}, Gupta et al. \cite{ContinualPre-TrainingofLarge}, EcomGPT-CT\cite{Ecomgpt}, QUERT\cite{quert}, Qin et al. \cite{Recyclable}, Mehta et al. \cite{Anempirical}, Cossu et al. \cite{Continualpre-trainingmitigates}, Li et al. \cite{examining}
                        },
                        color=cyan!100, fill=cyan!15, ultra thin, text=black, tier=Method
                    ]
                ]
                [Continual Temporal Domain Pretraining \cref{sec:continual_temporal_domain_pretraining}, color=cyan!100, fill=cyan!15, very thick, text=black, tier=Task, text width=3.0cm
                    [ 
                        {
                            ECONET\cite{econet}, Zhao et al. \cite{set}, TimeLMs \cite{timelms}, Lazaridou et al. \cite{mind}, Röttger et al. \cite{temporaladaptation}, Luu et al. \cite{timewaits}
                        },
                        color=cyan!100, fill=cyan!15, ultra thin, text=black, tier=Method
                    ]
                ]
                [Continual Language Domain Pretraining \cref{sec:continual_language_domain_pretraining}, color=cyan!100, fill=cyan!15, very thick, text=black, tier=Task, text width=3.0cm
                    [ 
                        {
                            PP-TF\cite{Exploringcontinual}, Ibrahim et al. \cite{simple}, CLL-CLIP \cite{embracing}, Gogoulou et al. \cite{continuallearning}, Lifelong-MoE \cite{Lifelonglanguagepretraining}
                        },
                        color=cyan!100, fill=cyan!15, ultra thin, text=black, tier=Method
                    ]
                ]
            ]
            [\footnotesize Continual Finetuning \cref{sec:continual_finetuning}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black
                [\footnotesize Task Specific, color=lightcoral!100, fill=lightcoral!15, very thick, text=black
                    [Continual Text Classification \cref{sec:continual_text_classification}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black, tier=Task, text width=3.0cm
                        [
                            {
                                Chen et al. \cite{chen2018lifelong}, 
                                B-CL \cite{ke2021adapting}, 
                                CLASSIC \cite{ke2021classic}, 
                                Paul et al. \cite{paul2022class}, 
                                DR-EMR \cite{vijayaraghavan2021lifelong}, 
                                CRN \cite{bai2022incremental}, 
                                SCN \cite{liu2023class}, 
                                InfoCL \cite{song2023infocl}, 
                                IDBR \cite{huang2021continual}, 
                                CCFI \cite{hua2021hyperparameter}, 
                                EPI \cite{wang2023rehearsal}, 
                            },
                            color=lightcoral!100, fill=lightcoral!15, ultra thin, text=black
                        ]
                    ]
                    [Continual Named Entity Recognition \cref{sec:continual_named_entity_recognition}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black, tier=Task, text width=3.0cm
                        [
                            {
                                Shen et al. \cite{shen2019progressive}, KCN \cite{cao2020incremental}, ExtendNER \cite{monaikul2021continual}, KD+R+K \cite{yu2021lifelong}, Wang et al. \cite{wang2022few}, L\&R \cite{xia2022learn}, CFNER \cite{zheng2022distilling}, OCILNER \cite{ma2023learning}, SpanKL \cite{zhang2023neural}, CPFD \cite{zhang2023continual}
                            },
                            color=lightcoral!100, fill=lightcoral!15, ultra thin, text=black
                        ]
                    ]
                    [Continual Relation Extraction \cref{sec:continual_relation_extraction}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black, tier=Task, text width=3.0cm
                        [
                            {
                                CEAR\cite{CEAR}, SCKD\cite{SCKD}, CRL\cite{CRL}, EMAR\cite{EMAR}, RP-CRE\cite{RPCRE}, FEA\cite{FEA}, KIP-Framework\cite{KIP}, CRECL\cite{CRECL}, CPL\cite{CPL}, ACA\cite{ACA}, ERDA\cite{ERDA}
                            },
                            color=lightcoral!100, fill=lightcoral!15, ultra thin, text=black
                        ]
                    ]
                    [Continual Machine Translation \cref{sec:continual_machine_translation}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black, tier=Task, text width=3.0cm
                        [
                            {
                                Cao et al. \cite{cao2021continual}, 
                                Shao et al. \cite{shao2022overcoming}, 
                                Khayrallah et al. \cite{khayrallah2018regularized}, LFR-CM and LFR-OM \cite{gu2022continual}, Liu et al. \cite{liu2023continual}, Garcia et al. \cite{garcia2021towards}, Huang et al. \cite{huang2022entropy}, Zhang et al. \cite{zhang2022clle}
                            },
                            color=lightcoral!100, fill=lightcoral!15, ultra thin, text=black
                        ]
                    ]
                ]
                [\footnotesize Task Agnostic, color=lightcoral!100, fill=lightcoral!15, very thick, text=black
                    [Continual Instruction-Tuning \cref{sec:continual_instruction_tuning}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black, tier=Task, text width=3.0cm
                        [
                            {
                                Jin et al. \cite{jin2021learn}, 
                                Peng et al. \cite{bohaoscalable},
                                O-LoRA \cite{wang2023orthogonal}, 
                                InsCL \cite{wang2024inscl},  
                                CTR \cite{ke2021achieving}, DMEA \cite{qin2023lifelong}, Liang et al. \cite{liang2023prompts}, LAMOL \cite{sun2019lamol}, LFPT5 \cite{qin2021lfpt5}, PCLL \cite{zhao2022prompt}, SCLL \cite{luo2023mitigating}, Ren et al. \cite{ren2024analyzing}
                            },
                            color=lightcoral!100, fill=lightcoral!15, ultra thin, text=black
                        ]
                    ]
                    [Continual Knowledge Editing \cref{sec:continual_knowledge_editing}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black, tier=Task, text width=3.0cm
                        [
                            {
                                GRACE\cite{GRACE}, T-Patcher\cite{TPatcher}, SLAG\cite{SLAG}, WilKE\cite{WilKE}
                            },
                            color=lightcoral!100, fill=lightcoral!15, ultra thin, text=black
                        ]
                    ]
                    [Continual Alignment \cref{sec:continual_alignment}, color=lightcoral!100, fill=lightcoral!15, very thick, text=black, tier=Task, text width=3.0cm
                        [
                            {
                            Personal privacy
                                CPPO \cite{zhangcppo}, COPR \cite{zhang2024copr}, Lin et al. \cite{lin2023mitigating}, Zhao et al. \cite{zhao2023learning}, Zhan et al. \cite{zhan2023removing}, Lermen et al. \cite{lermen2023lora}, Qi et al. \cite{qi2023fine}
                            },
                            color=lightcoral!100, fill=lightcoral!15, ultra thin, text=black
                        ]
                    ]
                ]
            ]
        ]
        [\footnotesize External Knowledge \cref{sec:external_knowledge}, color=lightgreen!100, fill=lightgreen!15, very thick, text=black 
            [Retrieval-Based Lifelong Learning \cref{sec:retrieval_based_lifelong_learning}, color=lightgreen!100, fill=lightgreen!15, very thick, text=black, tier=Task, text width=3.0cm
                [
                    {
                        RAG\cite{knowledge-intensivenlp}, DPR\cite{Densepassage}, IRCOT\cite{Interleavingretrievalwith}, ToC\cite{Treeofclarifications}, FLARE\cite{Activeretrievalaugmented}, Self-RAG\cite{Self-rag}
                    },
                    color=lightgreen!100, fill=lightgreen!15, ultra thin, text=black, tier=Method, 
                ]
            ]
            [Tool-Based Lifelong Learning \cref{sec:tool_based_lifelong_learning}, color=lightgreen!100, fill=lightgreen!15, very thick, text=black, tier=Task, text width=3.0cm
                [
                    {
                        Chameleon \cite{lu2024chameleon}, Confucius \cite{gao2024confucius}, Toolformer \cite{schick2024toolformer}, GPT4Tools \cite{yang2024gpt4tools}, ToolAlpaca \cite{tang2023toolalpaca}, APIBench \cite{patil2023gorilla}, ToolBench \cite{qin2023toolllm}
                    },
                    color=lightgreen!100, fill=lightgreen!15, ultra thin, text=black, tier=Method, 
                ]
            ]
        ]
    ]
\end{forest}
